Risk aversion in flexible electricity markets

Flexibility options, such as demand response, energy storage and interconnection, have the potential to reduce variation in electricity prices between different future scenarios, therefore reducing investment risk. Moreover, investment in flexibility options can lower the need for generation capacity. However, there are complex interactions between different flexibility options. In this paper, we investigate the interactions between flexibility and investment risk in electricity markets. We employ a large-scale stochastic transmission and generation expansion model of the European electricity system. Using this model, we first investigate the effect of risk aversion on the investment decisions. We find that the interplay of parameters leads to (i) more investment in a less emission-intensive energy system if planners are risk averse (hedging against CO2 price uncertainty) and (ii) constant total installed capacity, regardless of the level of risk aversion (planners do not hedge against demand and RES deployment uncertainties). Second, we investigate the individual effects of three flexibility elements on optimal investment levels under different levels of risk aversion: demand response, investment in additional interconnection capacity and investment in additional energy storage. We find that that flexible technologies have a higher value for risk-averse decision-makers, although the effects are nonlinear. Finally, we investigate the interactions between the flexibility elements. We find that risk-averse decision-makers show a strong preference for transmission grid expansion once flexibility is available at low cost levels.

==> nomenclature.tex <==
\makenomenclature
\mbox{}

\nomenclature[A]{$I$}{\hspace{1em} Technology}
\nomenclature[A]{$M$}{\hspace{1em} Month}
\nomenclature[A]{$N,\mathit{NN}$}{\hspace{1em} Node}
\nomenclature[A]{$\mathit{HR}(I)$}{\hspace{1em} Hydro reservoirs as subset of I}
\nomenclature[A]{$S$}{\hspace{1em} Scenario}
\nomenclature[A]{$\mathit{SEC}$}{\hspace{1em} Industry sector}
\nomenclature[A]{$\mathit{PSP}(I)$}{\hspace{0.5em} Pump storage plants as subset of I}
\nomenclature[A]{$T$}{\hspace{1em} (Representative) hours}
\nomenclature[A]{$Y$}{\hspace{1em} Year}
\nomenclature[B]{$\mathit{CAP}_{i,n,y}$}{\hspace{0em} Confidence level on CVar}
\nomenclature[B]{$\alpha$}{\hspace{1em} Confidence level on CVar}
\nomenclature[B]{$\eta_i$}{\hspace{1em} Efficiency rate of a generation technology}
\nomenclature[B]{$\rho_s$}{\hspace{1em} Probability of scenario s}
\nomenclature[B]{$\omega$}{\hspace{1em} Weight on CVar}
\nomenclature[B]{$\mathit{AF}_{i,n,t,y}$}{\hspace{0.1em} Availability factor for  conventional and renewable generation capacities}
\nomenclature[B]{$\mathit{CX}_{i,n,y}$}{\hspace{0.6em} Annualised investment costs power generation capacity [€$/MW_{el}$]}
\nomenclature[B]{$\mathit{CY}_{n,nn,y}$}{\hspace{0em} Annualised investment costs net transfer capacity [€$/MW_{el}$]}
\nomenclature[B]{$\mathit{CZ}_{y}$}{\hspace{1em} Annualised investment costs PSP capacity [€$/MW_{el}$]}
\nomenclature[B]{$D_{n,t,y,s}$}{\hspace{0.6em} Electricity demand [$MWh_{el}/h$]}
\nomenclature[B]{$\mathit{DF}_{y}$}{\hspace{1em} Discounting factor}
\nomenclature[B]{$\mathit{VC}_{i,n,y,s}$}{\hspace{0em} Variable generation costs [€$/MWh_{el}$]}
\nomenclature[B]{$\mathit{VOLA}_{sec,n,y}$}{\hspace{0em} Value of lost adequacy [€$/MWh_{el}$]}
\nomenclature[B]{$X^{max}_{i,n}$}{\hspace{1em} Upper limit for generation capacity investments [$MW_{el}$]}
\nomenclature[B]{$Z^{max}_{n}$}{\hspace{1em} Upper limit for storage capacity investments [$MW_{el}$]}
\nomenclature[C]{$\zeta$}{\hspace{1em} Value at risk}
\nomenclature[C]{$a_s$}{\hspace{1em} Auxiliary variable for CVaR}
\nomenclature[C]{$\mathit{cvar}$}{\hspace{1em} Conditional value at risk}
\nomenclature[C]{$g_{i,n,t,y,s}$}{\hspace{0.5em} Electricity generation [$MWh_{el}/h$]}
\nomenclature[C]{$\mathit{IC}$}{\hspace{1em} Total first-stage investment costs [€]}
\nomenclature[C]{$\mathit{OC}$}{\hspace{1em} Total second-stage operation costs [€]}
\nomenclature[C]{$sl_{i,n,t,y,s}$}{\hspace{0.3em} Storage level of PSP [$MWh_{el}$]}
\nomenclature[C]{$\mathit{TC}$}{\hspace{1em} Total system costs [€]}
\nomenclature[C]{$x_{i,n,y}$}{\hspace{1em} Investments in electricity generation capacity [$MW_{el}$]}
\nomenclature[C]{$y_{n,nn,y}$}{\hspace{1em} Investments in net transfer capacity [$MW_{el}$]}
\nomenclature[C]{$z_{psp,n,y}$}{\hspace{0.8em} Investments in pump storage capacity [$MW_{el}$]}

\printnomenclature
